The Bending of C$_3$: Experimentally Probing the $l$-type Doubling and Resonance

C$_3$, a pure carbon chain molecule that has been identified in different astronomical environments, is considered a good probe of kinetic temperatures through observation of transitions involving its low-lying bending mode ($\nu_2$) in its ground electronic state. The present laboratory work aims to investigate this bending mode with multiple quanta of excitation by combining recordings of high resolution optical and infrared spectra of C$_3$ produced in discharge experiments. The optical spectra of rovibronic (A $^1\Pi_u -$ X $^1\Sigma_g^+$) transitions have been recorded by laser induced fluorescence spectroscopy using a single longitude mode optical parametric oscillator as narrow bandwidth laser source at the University of Science and Technology of China. 36 bands originating from X(0$v_2$0), $v_2 = 0-5$, are assigned. The mid-infrared spectrum of the rovibrational $\nu_3$ band has been recorded by Fourier-transform infrared spectroscopy using a globar source on the AILES beamline of the SOLEIL synchrotron facility. The spectrum reveals hot bands involving up to 5 quanta of excitation in $\nu_2$. From combining analyses of all the presently recorded spectra and literature data, accurate rotational parameters and absolute energy levels of C$_3$, in particular for states involving the bending mode, are determined. A single PGOPHER file containing all available data involving the X and A states (literature and present study) is used to fit all the data. The spectroscopic information derived from this work enables new interstellar searches for C$_3$, not only in the infrared and optical regions investigated here but also notably in the $\nu_2$ band region (around 63 cm$^{-1}$) where vibrational satellites can now be accurately predicted. This makes C$_3$ a universal diagnostic tool to study very different astronomical environments, from dark and dense to translucent clouds.

==> name.tex <==

\section{Experimental methods} \label{sec:expt}

\subsection{Optical Spectroscopy}

The optical spectroscopic study of the \ax transition of \ccc has been performed  between 380 to 410 nm at the University of Science and Technology of China by using a laser induced fluorescence (LIF) setup that has been described in \citet{Zhang2017,Zhang2018,Zhang2020}. 
In this experimental set-up, \ccc molecules are produced in a pulsed DC discharge nozzle using two flat-top stainless steel electrodes \citep{Motylewski1999}. 
A gas mixture of 0.3\,\% acetylene (C$_2$H$_2$) diluted in argon is introduced into the nozzle by a General Valve (Series 9, 0.5 mm orifice). %\mam{if the expansion is planar, does it means there is a slit somewhere?}
High voltage pulses ($\simeq -2000$\,V, 20\,\textmu s, 10\,Hz) are applied to one of the electrodes while the other is grounded in order to produce an intense pulsed plasma.
The plasma containing \ccc molecules is then expanded and adiabatically cooled by collisions with the buffer gas. About 10\,mm downstream, the molecular beam is crossed perpendicularly by a laser beam. 
The right angle is chosen in order to suppress the Doppler broadening in the recorded spectra. Fluorescent emission from laser excited \ccc molecules is collected by a lens system perpendicular to the laser beam, guided into a grating spectrometer (Zolix, 0.5\,m) and then detected by a photomultiplier tube (Hamamatsu, R928). 

A home-built single-longitude-mode optical parametric oscillator (SLM-OPO) is employed as the laser source \citep{Zhang2017:note}. In the present study, the signal output of the OPO is frequency-doubled in a KDP (KH$_ 2 $PO$ _4 $) crystal to obtain tunable radiation between 350 and 450\,nm. A small portion ($\sim$ 5\,\%) of the OPO signal output is injected into a wavelength meter (High Finesse, WS7-60) for calibration. The wavelength meter is calibrated with a stabilized He-Ne laser, providing an absolute frequency accuracy of $\sim 0.002$\,\wn for the laser source.

Special care had to be taken in the measurement of the relatively weak hot vibronic bands. This is because in the supersonic jet the population of an excited vibrational state is much lower than that in the $v = 0$ state and, in most cases, the hot bands are overlapped with stronger fundamental vibronic bands. To overcome these difficulties, the spectrometer is used as a narrow band pass filter which helps selecting fluorescence of the hot bands from other overlapping bands. 
As the fluorescence emission from different upper states often results in different dispersion spectra, and since the bandpass of the monochromator is extremely narrow ($\sim$ 0.5 nm), it thus becomes possible to only detect the fluorescence emission from upper states involving specific GS hot bands. This was realized by selecting a dispersion wavelength of the monochromator corresponding to the fluorescence from the upper electronic state (itself optically-pumped from vibrationaly excited states of the \xt state) to the lowest allowed vibrational level of the GS.

A laser excitation spectrum is recorded by measuring the fluorescence intensity as a function of the continuously tuned laser wavelength. 
This technique yields a very good signal-to-noise (S/N) ratio and a spectral resolution of $\sim$\,0.02\,\wn (corresponding to a resolution power of $\sim$\,1,200,000) for the strong bands. Based on the line width of the rovibronic transitions, the accuracy of the extracted line positions from our spectra can confidently be assumed to be of about 0.002\,\wn for the bands arising from $v''_2 = 0, 1$ in the ground electronic state [with the exception of the \at(000)--\xt(000) band for which a 0.005\,\wn uncertainty is used] and 0.005\,\wn for the other hot bands (with $v''_2 \geq 2$). Absolute frequency accuracies may be subject to small shifts because of combining spectra from different wavelength regimes that are recorded in different experimental setups, but comparison with previous studies \citep[e.g.,][]{Gendriesch2003,Schmuttenmaer1990, Tokaryk1997} allows for reliable calibration (see later in section \ref{sec:methodo}).
 

\subsection{Infrared Spectroscopy}
 
The absorption spectrum of \ccc has been recorded in the $\nu_3$ asymmetric stretch region (around $2000$\,\wn /  5\,\textmu m) using an experimental set-up available on the AILES beamline of synchrotron SOLEIL and previously used to investigate the far-IR spectra of various reactive species \citep[see][]{Martin-Drumel2011, Martin-Drumel2012, Martin-Drumel2014}. The schematic representation of the discharge set-up together with its implementation on the AILES beamline is given in Fig. 1 of \citet{Martin-Drumel2011}. We briefly describe in this paper the main characteristics of the set-up and the discharge conditions we used to optimize the signal of \ccc. The discharge cell consists of a 1.1\,m long Pyrex tube (13\,cm inner diameter) equipped with multipass optics (White-type) allowing for 24\,m of absorption pathlength. The cell is connected under vacuum to a Bruker Fourier-transform (FT) IR spectrometer and separated from it by two wedged \ce{CaF2} windows. A total of seven cell inlets are used: two are connected to the two water-cooled electrodes (separated by 70\,cm), four allow for gas injection (buffer gas or sample) at different locations in the cell, and one located at the center of the cell is connected to a vacuum system (roots blower).
To probe the positive column of the plasma, one of the electrodes is connected to the high voltage while the second is grounded.
In the present work, \ccc is synthesized using a discharge of He (injected both through the electrodes and through the two gas inlets closest to the multipass optics) seeded with a small amount of \ce{CH4} (injected using the inlets located closer to the center of the cell). 


Under our experimental conditions, we find that the abundance of \ccc is very sensitive to both the discharge current and the pressure of \ce{CH4} precursor. 
To optimize the production of \ccc, we  use a rapid scan optical fiber spectrometer (Ocean Optics) to monitor the 4051\,\AA\ emission band. The \ce{CH4} pressure is slowly increased until reaching the maximum of the visible emission while the discharge current is adjusted as well. In the optimum conditions, about 1\,A of current (at 1\,kV DC) is driving the discharge through  ballast resistors for a total of 100\,$\Omega$. A total pressure of about 1\,mbar of a mixture of \ce{CH4} seeded in He is injected in the cell and a continuous flow of gas is maintained using a 250\,m$^{3}$/h roots blower. 
To record the absorption spectra in the 5\,\textmu m region, we use the globar internal source of the Bruker FTIR installed on the AILES beamline of the SOLEIL synchrotron, a CaF$_2$ beamsplitter, and an Indium Antimonide (InSb) detector. These experimental conditions, together with the use of a bandpass optical filter, limit the bandwidth of our acquisition to the 1850--2100\,cm$^{-1}$ range. The unapodized spectral resolution is set to 0.004\,cm$^{-1}$ and 138 scans are co-added. Despite the effort to optimize the synthesis of \ccc in our cell and reduce the noise floor, the most intense lines of our spectra correspond to only about 5\,\% of signal absorption resulting in a SNR of 10 at best. 

Aside from \ccc, intense absorption lines of CO (possibly produced by reaction with residual H$_2$O) belonging to the $\Delta v = 1$ sequences (with $v'' =0-14$, the 4 -- 3 band being the strongest one) of the species in its electronic GS have been observed over the full spectral range covered in this study (Fig. S1 in the \esi). Even though these series of intense lines hindered identification of weaker series of \ccc lines, they enabled spectral calibration by comparison with the accurate wavenumbers values from \cite{Wappelhorst1997,Schneider1990a, Schneider1990b}. 
After calibration, the frequency accuracy is estimated for each  \ccc line  based on its full-width at half-maximum and signal-to-noise ratio \citep{Davis2001:FT} and ranges from 0.0005\,\wn to 0.006\,\wn.
The rotational contour of the CO bands also allows for estimation of its rotational temperature (see Fig. S2 in the \esi) from comparison with simulations using the \pgo software \citep{Western2017}. Under our experimental conditions, a rotational temperature of 500\,K is found in each CO band. Since the observation of CO hot bands is limited by the spectral coverage rather than the band population, no vibrational temperature value can be asserted. 
Besides CO lines, a few weak transitions of the fundamental bending mode $\nu_2$ of H$_2$O 
have also been detected \citep{Loos2017} and several lines have been assigned to the R branch of the fundamental $\nu_3$ band of C$_2$H in the 1860--1895\,\wn range \citep{Kanamori1987} (Fig. S1).


\subsection{Methodology \label{sec:methodo}}

As mentioned previously, the $\nu_2$ vibrational band lies in the far-IR region and is significantly weaker than the $\nu_3$ band \citep{Jensen1992}; for these reasons, it remains challenging to measure the hot band sequences involving $v_2$ which would provide vibrational energies in the $v_2$ progression. 
Alternatively, such information can be derived from a combined rovibronic and rovibrational analysis of bands involving various quanta of $\nu_2$ excitation in the electronic GS. This approach has been used in the present study exploiting \ccc spectra in the optical and mid-infrared region. 

Initial analyses of optical and infrared data have been performed independently, mostly exploiting combination differences.
Subsequently, all literature and newly measured rotationally-resolved transitions have been imported into the \pgo software \citep{Western2017} which has been used successfully  to analyze specific bands of \ccc  previously \citep[][]{Saha2006, Haddad2014, Schroeder2018, Zhang2021}.
Some features of this software have proven particularly powerful in the present study. First, all assignments can be treated as separate input files (for instance, a file per band) hence easing the treatment of large datasets. Then, the software allows for a relatively straightforward simultaneous treatment of rovibrational and rovibronic data. Last but not least, graphical representations of residuals, simulated bands, and term values plots is an invaluable tool to refine assignments and detect perturbations.
We thus perform a combined fit using \pgo of the presently recorded data together with all available rovibronic (\ax only) and rovibrational (all known bands in the \xt state) literature data allowing for the most complete spectroscopic description of the \ccc molecule to date. %, using an effective Hamiltonian,


\subsection{Spectroscopy of \ccc} \label{sec:spectro}

As already mentioned in the introduction,  detailed descriptions of the spectroscopy of \ccc can be found in \citet{Gausset1965} and \citet{Rousselot2001}; here we recall some aspects pertinent to this work.

In the \xs electronic GS, as a result of the presence of a doubly-degenerate bending vibration, the species exhibits to \textit{l}-type doubling. States with $v_2 > 0$ are split into multiple \textit{l}-states, with $l$ the vibrational angular momentum, such that \textit{l} = $v$, $v - 2$, ..., 0 or 1. Because the \ccc bending frequency is unusually small ($\omega_2 \sim 63$ \wn), the $l$-type doubling is unusually large.
In addition, the \as electronic state is subject to Renner-Teller coupling, splitting the $v_2$ bending states into $K= \abs{l \pm \Lambda}$ components, where $K$ is the total vibronic angular momentum and $\Lambda$ the projection of the electronic orbital angular momentum onto the molecular axis of the molecule. Again, the very small bending frequency yields significant effects on \ccc spectroscopy, here resulting in a large Renner-Teller interaction.
A typical representation of splittings for the bending mode of linear molecules experiencing Renner-Teller interaction is given in Fig. 9 of \cite{Gausset1965}. 


Because \ccc is linear, thus centrosymmetric, and contains identical nuclei of zero spin, all the antisymmetric levels have zero weight by spin statistics. In other words, half of the rotational levels is missing. For example, for $\Sigma^+_g$ states, only even-$J$ ($e$) levels exist while for a $\Sigma^+_u$ state, only odd-$J$ ($f$) levels exist. For other states, all $J$ levels exist but with alternate $e$/$f$ parity. 

In the following, each vibronic level is labeled $M$($v_1$, $v_2$, $v_3$) $N_s$ where $M$ is the electronic state (\xt\ or \at), $v_i$ ($i=1-3$) refers to the quanta of excitation in each vibrational mode, $N$ is the Greek letter associated to the $K$ quantum number, and $s$ the symmetry of the state ($g$ or $u$). For instance, the \xt(0,2,0) $\Delta_g$ state corresponds to the $v''_2=2$, $K=l=2$ vibrational level in the \xs electronic state; the \at(0,2,0) $\Phi_u$ state corresponds to the $v'_2=2$, $K=3$ (hence $l=2$) vibrational level in the \as electronic state. When discussing rovibrational transitions in the \xs\ state, the \xt\ is often omitted.


\section{Results and discussion} \label{sec:res}
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\textwidth]{Figures/plot_C3egy_2col_txt.pdf}
    \caption{Schematic vibrational energy level diagram of \ccc together with optical (in dashed lines) and infrared (in plain lines) bands observed in this work. Energy levels are represented with increasing quanta of excitation in $v_2$ from left to right. Energies are from the combined fit performed in this work. Only the levels involved in bands observed in the present study are plotted, with the exception of the (0$v'_2$0) levels, $v'_2=0-5$, in the \as state for which all levels included in the combined fit are shown. Transitions in the same color arise from the same (0$v''_2$0) lower state.   }
    \label{fig:C3bands}
\end{figure*}

Our rovibronic and rovibrational sets of data are extremely complementary as illustrated in Fig. \ref{fig:C3bands}, allowing to retrieve both accurate energies and spectroscopic constants for states involving $v''_2 = 0-5$. 
With regard to the (0$v''_2$0), $v''_2=0-5$, vibrational levels in the \xs state, the single fundamental piece of information not accessible using our combined data set alone is the energy of the \xt(010) $\Pi_u$ state (see Fig. \ref{fig:C3bands}); a value that has fortunately been determined accurately by \citet{Schmuttenmaer1990}.



\subsection{Optical data} \label{sec:optical RA}

\begin{figure*}[th!]
	\begin{center}
		\includegraphics[width=2\columnwidth]{Figures/plot_C3_A-X_txt.pdf}
		\caption{Overview of the electronic spectra of \ccc recorded in this work. \textit{Top traces:} Experimental spectra. \textit{Bottom traces:}  \pgo simulation (at thermal equilibrium and rotational temperatures reflecting each experimental band, from 20 to 150\,K; see Table S1 in the \esi). Intensities are in arbitrary units and the ratio between simulated bands is adjusted to reflect the experimental traces. Each simulated band is color coded according to the hot band of $\nu_2$ involved in the \xs state (the color sequence ranges from purple to red and the color coding is the same as in Fig. \ref{fig:C3bands}). Bands involving perturber states are plotted in the same color as the band they perturb. At this scale, bands arising from the same upper state and ending onto different GS levels, $e.g.$, \xt(020) $\Sigma_g^+$ and \xt(020) $\Delta_g$, are overlapping. Zoom onto the \at(000)--\xt(020) (highlighted by a star symbol on the figure) and \at(010)--\xt(030) $\Sigma_g^- -\Pi_u$ and $\Sigma_g^- -\Phi_u$ (highlighted by a triangle) band systems are presented in Fig. \ref{fig:AX000-020} and \ref{fig:AX010-030}, respectively.
		}
		\label{Fig:C3_A-X_full}
	\end{center}
\end{figure*}

\input{Tables/AssignedBandsOptical}

In the 24300--26500\,\wn region, 36 \ax vibronic bands have been recorded by LIF spectroscopy as summarized in Table~\ref{tab:OpticBandsDataset} and visible on Fig. \ref{Fig:C3_A-X_full}. Of these, 19 are reported for the first time. 
The strongest bands in the optical spectra belong to transitions arising from the \xt(000) state (Fig. \ref{Fig:C3_A-X_full}).
The \pgo software allows to estimate the rotational temperature of each band; it ranges for 20 to 150\,K (see Table S1 in the \esi). Typical linewidths reproducing the experimental spectra range from 0.02 \wn to 0.04 \wn. 
The present measurements are in good agreement with band values previously reported in the literature and often provide more accurate frequencies (see Table S2 in the \esi).  
Thanks to the relatively low rotational temperature combined with the high resolution resulting in well-resolved features, assignments of the new bands are relatively straightforward. Several bands appear heavily perturbed, in particular those involving the \at(020) $\Pi^{(-)}$ and \at(040) $\Pi_u^{(+)}$ states. 


In the \at(000)--\xt(020) band region, we assign for the first time transitions involving the u$\Sigma_u$ and u$P_u$ upper state perturbers, previously only observed in the \at(000)--\xt(000) band region \citep{McCall2003, Zhang2005, Haddad2014}. In total, 22 transitions have been assigned in the bands involving \xt(020): 11 in the u$\Sigma_u$--$\Sigma_g ^+$ band (P-, Q-, R-branch; although the single Q-branch assignment remains tentative), 5 in the u$P_u$--$\Sigma_g^+$ band (P- and R-branch), and 6 transitions in the u$\Sigma_u$--$\Delta_g$ band (P- and R-branch). No transitions were observed for the u$P_u$--$\Delta_g$ branch. Figure \ref{fig:AX000-020} presents an overview of this band system with the sub-bands highlighted in various colors. These transitions are predicted by \pgo without setting up a transition moment for the corresponding bands (Table S1 in the \esi).
One can notice that the simulated intensities of the perturber transitions do not perfectly reproduce the experimental spectrum on that figure (in particular for the $u\Sigma_u$--$\Delta_g$ band intensity is overestimated); we assume that some intensity perturbations are not properly taken into account. The agreement in line position, however, is quite satisfactory.
The present assignments thus comfort the assignment of the perturber lines  observed in the \at(000)--\xt(000) region.
It is also worth noticing that, on Figure \ref{fig:AX000-020}, the R-branches of the $\Pi_u$--$\Sigma_g ^+$ and $\Pi_u$--$\Delta_g$ bands (above 24545\,\wn) appear stronger in the experimental spectrum than on the simulation, and stronger than the Q-branches (the strongest features around 24540 \wn). Since no rotational temperature allows to properly reproduce such intensity ratio, this intensity difference is either the result of an experimental adjustment or some discrepancy in the model that does not properly apply to the present band system.
For the $\Pi_u$--$\Delta_g$ band, half of the $\Delta_g$ levels, with even $J''$ values, was previously observed by \citet{Gausset1965}. This peculiarity has led the authors to a better understanding of the $l$-uncoupling in the ground electronic state of \ccc. In the present study, we are able to assign transitions involving both even and odd $J''$ values. The transitions involving odd $J''$ values appear about 5 times weaker on the experimental spectrum than predicted using \pgo, and are thus significantly weaker than those involving even $J''$ values, which may explain why they remained unobserved thus far.  


\begin{figure}[th!]
    \centering
    \includegraphics[width=\columnwidth]{Figures/plotC3_AX_000-020.pdf}
    \caption{Overview of the \at(000)--\xt(020) band system observed around 24540 \wn (left panel), zoom onto a portion of the spectral range (right panel) and comparison with a \pgo simulation at 70\,K (lower traces). In the simulation, transitions within each sub-band are plotted in various colors. For the $\Pi_u$--$\Delta_g$ band, transitions involving even and odd $J''$ values ($e$ and $f$ levels in the lower state) are plotted in two shades of green with the intensity of the simulated $f$ symmetry divided by a factor 5 compared to the \pgo simulation. For the transitions involving the perturber states in the \as state, no scaling factor was used for the intensities as we could not define one that would be valid over the full spectral range.}
    \label{fig:AX000-020}
\end{figure}


Three $\Delta K= - 2$ bands have been observed in this study, namely \at (010) -- \xt (030) $\Sigma_g^-$--$\Phi_u$ (P-, Q-, and R-branches, Figure \ref{fig:AX010-030}), \at (000) -- \xt (040) $\Pi_u$--$\Gamma_g$ (P- and Q-branches, tentative assignments in the R-branch, see Figure S3 in the \esi), and \at (020) -- \xt (040) $\Pi_u^{(-)} - \Gamma_g$ (P- and Q-branches, Figure S4 in the \esi). To our knowledge, it is the first time that these transitions are observed for the \ax band.
These bands are spectrally intertwined with the corresponding $\Delta K= \pm 1$ bands arising from the same upper state and their intensity is properly predicted by \pgo  by perturbation (i.e., even though no transition moment is used to predict them, see Table S1 in the \esi). These nominally forbidden transitions appear quite strong both on the simulation and the experimental trace, as visible on Figure \ref{fig:AX010-030}. We note, however, that again the R-branches of both bands (located above 24,605\,\wn) are stronger on the experimental spectrum than predicted by the simulation. 


\begin{figure}[th!]
    \centering
    \includegraphics[width=\columnwidth]{Figures/plotC3_AX_010-030.pdf}
    \caption{Overview of the (010)-\xt(030) $\Sigma_g^- -\Pi_u$ and $\Sigma_g^- -\Phi_u$ band system observed around 24600 \wn (left panel), zoom onto a portion of the spectral range (right panel) and comparison with a \pgo simulation at 150\,K (lower traces). In the simulation, transitions from the $\Delta K= -1$ band are in gray and those from the $\Delta K= -2$ band are highlighted in orange.}
    \label{fig:AX010-030}
\end{figure}



Two bands of the \at(010)--\xt(050) band system, namely the $\Delta_g$--$\Pi_u$ and $\Delta_g$--$\Phi_u$ bands, have been observed in this work (see Figure S5 in the \esi). Again, to the best of our knowledge, these bands are the first bands of the \ax transition probing the \xs (050) state at high resolution. A single band probing higher quanta of excitation in $\nu_2$ was previously reported in the literature, the \at(000)--\xt(060) $\Pi_u$--$\Sigma_g^+$ band for which Q-branches assignments were proposed by \citet{Merer1967}. In the present work, the spectral range where this band lies (around 24217\,\wn) has not been investigated and not other band involving the \xt (060) state has been observed, hence preventing assignments confirmation by combination differences. 
Additional figures showing overviews of all \ax bands observed in this study are reported in the \esi (Fig. S6--S17).


\subsection{Infrared data} \label{sec:IR RA}
\begin{figure*}[ht!]
	\begin{center}
		\includegraphics[width=2\columnwidth]{Figures/plot_C3_fullrange.pdf}
		\caption{Spectrum of \ccc in the 1850--2100 cm$^{-1}$ spectral range. \textit{Top trace:} Absorption spectrum presented in transmittance. The intense absorption lines of CO as well as the lines of \ce{H2O} and \ce{C2H} were removed from the experimental trace for clarity. \textit{Bottom trace:}  A 700 K \pgo simulation (at thermal equilibrium) of the $\nu_3$ band of \ccc and its hot bands involving up to five quanta of excitation in $\nu_2$. The hot band sequence is plotted in a color sequence ranging from purple to dark red. The simulation is normalized to the strongest transition of the fundamental $\nu_3$ band. The color coding is the same as in Fig. \ref{fig:C3bands}. 
		}
		\label{Fig:C3_Full}
	\end{center}
\end{figure*}

\input{Tables/AssignedBandsMIR}

The full FTIR absorption spectrum of \ccc recorded in this work is shown in Fig. \ref{Fig:C3_Full}. The intense absorption features from CO, H$_2$O, and C$_2$H have been removed from the experimental trace for clarity. 
The simulated spectrum given in the lower part of the figure is obtained using the \pgo software \citep{Western2017} using the band center and rotational constants obtained from our fit (see section \ref{sec:fit}), a Gaussian lineshape with a 0.005\,\wn width, and assuming a 700\,K rotational temperature (which was found to better reproduce the fundamental $\nu_2$ band; we note that this temperature is higher than that found for CO). The hot band sequence involving increasing values of $v''_2$ extends toward lower frequencies as visually indicated by the colored sequence. 
Fig. \ref{Fig:C3_Full} also illustrates the strong overlap of all the bands observed in this work which caused most of the difficulties in the assignment process. 
For example, the lines arising from the (051)--(050) bands span over most of the spectral region. Since they are weak and hindered by many other more intense lines, their assignment was challenging. 
In total,  18 rovibrational bands of \ccc have been observed in this study, 14 of them for the first time (see Table \ref{tab:MIRBandsDataset}).
A detailed account on this work and available literature of rovibrational data is available in Table S3 in the \esi. In this work, the assignment of the IR data was performed separately from the optical measurements presented in the previous sections and  strongly relied on the literature data (including optical studies).

The analysis of the (001)--(000) $\Sigma_u^+$--$\Sigma_g^+$, (011)--(010) $\Pi_g$--$\Pi_u$, and (021)--(020) $\Sigma_u^+$--$\Sigma_g^+$ and $\Delta_u$--$\Delta_g$ bands was rather straightforward  thanks  to  the  diode  laser  experiments  performed  by  \citet{Matsumura1988} and \citet{Kawaguchi1989}.  For all these bands, our observations are perfectly consistent with the literature measurements and allow for an extension of the dataset toward high-$J$ values (up to 55--60, see Table \ref{tab:MIRBandsDataset}). The frequency accuracy is slightly improved for the (001)--(000) and (011)--(010) bands (by up to a factor 2, with values as low as 0.0005 \wn) and similar for the (021)--(020) bands (see Table S3 in the \esi).
Our extended dataset and the use of $\Delta_2^{up}$($J$) allowed to identify local perturbations in the upper \xt(021) $\Delta_u$ levels manifold. Figure \ref{fig:020FigPerturbs} shows the diagrams of the first derivative of the second differences, $\Delta_2^{up}$($J$) values, calculated in the upper states. The highest shift occurs for the \xt(021) $\Delta_u$ $e$ manifold at $J'$ = 35 (the shift corresponds to about 10$\times$ the \ccc linewidth), and similar but smaller shift observed for the \xt(021)$f$ manifold. No notable level shifts are observed in (021) $\Sigma_g^+$ state. The  observed perturbations in the $\Delta_u$ state are likely caused by a Coriolis interaction with the \xt(19$^1$0) manifold, which mixes energy levels with $\Delta J$ = 0, e $\leftrightarrow$ e or f $\leftrightarrow$ f, and $\Delta$\textit{l} = odd. While the \xt(19$^1$0) state has not yet been detected in Stimulating Emission Pumping (SEP) measurements, observations of \xt(18$^0$0) at about 1993\,\wn puts the \xt(19$^1$0) state in the right energy range \citep{Northrup1990}.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=\columnwidth]{Figures/plot_020_perturb.pdf}
    \caption{Perturbation analysis of the \xt(021) $\Delta_u$ e and f  manifolds. }
    \label{fig:020FigPerturbs}
\end{figure}


We detected for the first time numerous infrared transitions involving the (031)--(030), (041)--(040), and (051)--(050) hot bands. The assignment procedure relied mainly on combination differences using the work of \citet{Gausset1965} (see the \esi for a detailed explanation on the procedure). 
As no combination differences were available for the (030) $\Phi_u$ state, we used the results of successive fits which included $l$-type resonance with the $\Pi$ state to secure the assignments. Further confirmation is obtained by ground state combination differences using the present optical data.
SEP data from \citet{Rohlfing1989:SEP} and \citet{Northrup1989}, despite their limited resolution, have provided crucial information on states for which little was known so far (vibrational energies and estimated $B$ values). In several cases, for example the (051)--(050) band manifold, this provided sufficient information to initiate an analysis.  %often permitted to initiate the analysis. 


\citet{Rohlfing1989:SEP}  reported the vibrational energy of the \xt(051) $\Pi_g$ state [2330.9(5)\wn] as well as an estimation of the rotational constants for the lowest $J$ values [$B$ = 0.4718(13)~cm$^{-1}$]. Using this information we started our analysis for the $\Pi$~$e$ and $\Pi$~$f$ states. Once $\Pi$ states were found (up to $J''$ = 40 for both $e$ and $f$ transitions), we used the $l$-type resonance to secure the assignments of $\Phi_g$--$\Phi_u$ and $\mathrm{H}_g$--$\mathrm{H}_u$ bands. 
The intensities of the P branches involving high $J$ values are very weak (red-end of our spectrum) and, as for the $\Delta$ states of (021), some Coriolis-type resonances seem to complicate the assignments. %A possible perturber could be \xt(0 22 0). 
Figs. S18--S23 in the \esi show the different infrared band manifolds observed in this study.

The rotational assignments proposed in this study are confirmed by the observation of several Q-branches, i.e., no shift by one or more quanta of $J$ is possible in the proposed assignments. Such a $Q$-branch is shown on Fig. \ref{fig:Q050} for the (051)--(050)  $\mathrm{H}_g$--$\mathrm{H}_u$ band, another example is provided for the (041)--(040)  $\Gamma_u$--$\Gamma_g$ band in Fig. S24 in the \esi. Overall, Q-branch transitions were observed, for both $e$ and $f$ levels, for the (011)--(010) $\Pi_g$--$\Pi_u$ [Q(1),Q(3)], (021)--(020) $\Delta_u$--$\Delta_g$ [Q(2), tentative], (031)--(030) $\Phi_g$--$\Phi_u$ [Q(3)--Q(6)], (041)--(040) $\Gamma_u$--$\Gamma_g$ [Q(4)--Q(7)], and (051)--(050) $\Phi_g$--$\Phi_u$ [Q(3)--Q(5), Q(6) tentative] and $\mathrm{H}_g$--$\mathrm{H}_u$ [Q(5)--Q(11)] bands.


\begin{figure}[ht!]
    \centering
    \includegraphics[width=\columnwidth]{Figures/Qbranch_051-050_txt.pdf}
    \caption[Q-branch in \xt(051)--\xt(050)  $\mathrm{H}_g$--$\mathrm{H}_u$ band]{Zoom onto the Q-branch of the \xt(051)--\xt(050)  $\mathrm{H}_g$--$\mathrm{H}_u$ band. \textit{Top trace:} experimental spectrum, in transmittance, after removal of CO, \ce{H2O}, and \ce{C2H} lines. \textit{Bottom trace:} \pgo simulations at 700 K (final set of parameters).}
    \label{fig:Q050}
\end{figure}


Once all the data were included in \pgo, we were also able to assign some transitions involving $\Delta l = \pm 2$ bands. 
An interesting feature of \pgo is that it predicts these transitions without inputting a corresponding transition moment for these nominally ``forbidden'' transitions (similarly to what was described previously for the electronic spectra). 
For the (021)--(020) bands, these $\Delta l = \pm 2$ bands are predicted with relatively low intensities; and only features with relatively poor SNR are observed on the experimental spectrum. Only tentative assignments have been made (7 for the $\Delta_u$--$\Sigma_g^+$ and 4 for the $\Sigma_u^+$--$\Delta_g$ band) and these are not included in the fit. 
For hot bands involving higher quanta of excitation in $\nu_2$, however, these predicted $\Delta l = \pm 2$ transitions have significant intensity, in particular for high $l$ values. Indeed, several features with reasonable SNR are observed on the spectrum as visible on Fig. \ref{fig:040-forbidden} for the (041)--(040) $\Gamma_u$--$\Delta_g$ band. Additional examples are provided in the \esi for the (031)--(030) $\Pi_g$--$\Phi_u$ and $\Phi_g$--$\Pi_u$ bands (Fig. S25) and the (041)--(040) $\Delta_u$--$\Gamma_g$ (Fig. S26).
These ``cross-ladder'' transitions (if we refer to levels of a given $l$ value for a specific state as a ladder) provide constraints on the energy difference between the various $l$ levels of the vibrational states for which they are observed.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=\columnwidth]{Figures/forbidden_041-040_txt.pdf}
    \caption{Zoom onto three consecutive R-branch transitions of the (041)--(040) $\Gamma_u$--$\Delta_g$ band. \textit{Top trace:} experimental spectrum, in transmittance, after removal of CO, \ce{H2O}, and \ce{C2H} lines. \textit{Bottom trace:} \pgo simulations at 700 K (final set of parameters,  normalized to the strongest transition of the fundamental $\nu_3$ band) where the $\Gamma_u$--$\Delta_g$ transitions are highlighted in green. The rest of the simulated transitions of the (041)--(040) bands visible in this range are plotted in shades of red while the other \ccc bands are simulated in gray.}
    \label{fig:040-forbidden}
\end{figure}


In the high frequency part of the spectrum, most of the transitions can be assigned to the \ccc molecule (see for instance figure \ref{fig:040-forbidden} and figure S27 in the \esi). Toward the lower end of the spectrum, however, many transitions remain unassigned. These transitions probably arise from the R-branches of the (061)--(060) bands but assigning this  spectrum has not been possible despite our best efforts, mainly because the signal-to-noise ratio is rather poor in that region and spectroscopic assignments are challenging on the basis on a single branch.


%\FloatBarrier
\subsection{Combined fit} \label{sec:fit}

\subsubsection{Dataset}
The unique feature of the present work is that it becomes possible to combine the optical and infrared data sets. Available data from the literature and the present work for the \ax rovibronic transition and all \xx rovibrational transitions are listed in Tables S2 and S3 in the \esi. These detailed tables contain the $J_\mathrm{max}$ values, frequency uncertainties used in the combined fit, and the frequency offset eventually applied to the data. All available (i.e., data with list of assignments provided in the literature) \ax data and rovibrational transitions in the electronic GS are included in the present fit at two exceptions. The first exception is the work of \citet{Schmidt2014} for which linelists are provided but it remains unclear to us if the reported frequencies are experimental or calculated. The second exception is the work of \citet{Balfour1994}, who reported the spectroscopic assignments for five \ax transitions of \ccc. One rovibronic band observed by \citet{Balfour1994}, namely the \at(020) -- \xt (000) $\Pi_u$--$\Sigma_g^+$ band, was re-investigated by \citet{Tokaryk1997} who proposed  a different spectroscopic assignment. In the present study, our assignments are in line with those of \citet{Tokaryk1997}. Additionally, we propose in this work an alternative spectroscopic assignment for the \at(002) -- \xt (000) $\Pi_u$--$\Sigma_g^+$ band compared to \citet{Balfour1994}. Finally, when performing the combined fit, we noticed that the spectroscopic assignments proposed by \citet{Balfour1994} in the \at(200) -- \xt (000) $\Pi_u$--$\Sigma_g^+$ band are incompatible with those of the \at(200) -- \xt (200) $\Pi_u$--$\Sigma_g^+$ from \citet{Merer1967}. Since assignments from \citet{Merer1967} have proven consistent with literature data for the other bands they reported, we decided only include the Merer values. 
There is no literature data able to confirm or infirm the spectroscopic assignments of the remaining two bands observed by \citet{Balfour1994}; at this stage we have chosen not to include these data in our fit.

As previously noted by \citet{Saha2006}, a serious difficulty arises in high resolution combination fits when rovibronic data are included from different light sources, as (small) spectral offsets are intrinsic to this approach; an issue that usually concerns rovibronic data.
This can be overcome by shifting the frequencies of one dataset by its offset value. It is often challenging, however, to determine which dataset presents an offset from the absolute transitions rest frequencies. The impact of this issue is relatively limited because only the absolute energy of the upper state is affected while the accuracy of the rotational constants and overall fit is not. In the present study, small offsets (typically of the order of several hundredths of a \wn)  are applied to several rovibronic datasets (see Table S2 for a detailed list of concerned data and offset values). We use the frequency offsets established by other authors from the literature when available (for instance, an offset of $+0.04$ \wn was determined for the data of \citet{Gausset1965} by \citet{Tanabashi2005}) for consistency reasons and when not available we determine these offsets ourselves. 
Overall, offsets values range from 0.02 to 0.12 \wn, hence the absolute energies in the \as state may be affected by these amounts. 

As much as possible, data are included in the fit at their experimental accuracy (see Table S2 for typical values for each dataset). When no frequency accuracy was provided, we assume a value based on the dispersion of the frequency from our best model. In some instances, the literature data are provided with an upper limit for the frequency error but the residuals from the fit show that this value is over-estimated. For example, the uncertainty on line frequency is assumed to be better than 0.01 \wn for the \at(000) -- \xt(000) transitions reported by \citet{Zhang2005} but the residuals from our fit show that the line accuracy is probably more of the order of 0.005 \wn; that value is thus used in the present fit.
It has proven challenging to treat such a large dataset for one molecule subject to clear perturbations with transitions significantly deviating from the fit. 
Transitions severely perturbed are excluded from the fit while transitions slightly diverging are kept in the fit but with an increased frequency error (hence a lower weight), typically by a factor 10, in order to maintain a global $5\sigma$ deviation for the combined fit. Overall, the dataset contains 4344 observations (2876 rovibronic and 1468 rovibrational transitions) including 2046 (1106 rovibronic and 940 rovibrational transitions) from this work. The full dataset is available as electronic files as part of the \esi (these files also contain the transitions not included in the present fit).


\subsubsection{Hamiltonian}
The \pgo Hamiltonian used for the combined fit is similar to the previous studies using \pgo on \ccc. One difference with the work of \citet{Haddad2014} is that we expressed the Hamiltonian in terms of the rotational angular momentum of the nuclear framework, $\mathbf{\hat{R}}$, in order to obtain energy levels and rotational constants comparable with most of the literature data. 
It is worth noting that the specific Hamiltonian used by the \pgo software differs from the conventional Hamiltonian for a linear molecule developed for instance by \citet{Yamada1985}.
The off-diagonal constants accounting for $l$-doubling are expressed as perturbation terms between two states, which results in several $q$ values for a given vibrational state instead of a more physically-relevant single one (see Table S4). For example, for the \xt(050) vibrational state there are three different $q$ values: one for the $\Pi$ state, and two defined as $\bra{\Pi_u}q\ket{\Phi_u}$ and $\bra{\Phi_u}q\ket{\mathrm{H}_u}$.
The resulting \pgo files together with details on their construction are provided in the \textbf{Supplementary Material}. 

The perturbation analysis for the \at(000)--\xt(000) band is carried out using the same effective Hamiltonian as reported in \citet{Haddad2014}, with the two perturbing $\Sigma$ and $P=1$ states identified in the literature treated as three perturbing states with the $e$ and $f$ levels of the  $P=1$ state treated separately. The resulting states are labeled u$\Sigma$, u$P_e$, and u$P_f$. As in \citet{Haddad2014}, the spin-spin interaction constant $\lambda$ was fixed to 0.1 \wn in the u$\Sigma$ state. Table S5 in the \esi presents the resulting constants in these perturbing states.


\subsubsection{Fit results}

A total of 340 parameters have been adjusted to reproduce the more than 4000 experimental data with a rms of 0.042 \wn and reduced standard deviation of 1.3. Figure \ref{fig:res} displays the residuals of the fit with a color coding based on the \xt($v_1v_2v_3$) state involved in the transition (the same as in Fig. \ref{fig:C3bands}). Overall, the fit is quite satisfactory. One can notice that the IR (021)--(020) transitions (in green, around observation \#200) are among those the least well reproduced by the fit as a result of severe perturbations in the state \xt(021) state.


\begin{figure}[ht!]
    \centering
    \includegraphics[width=\columnwidth]{Figures/residualsFit.pdf}
    \caption{Residuals of the combined fit. Transitions involving the \xt(0$v_2$0) vibrational state, with up to five quanta of excitation in $\nu_2$, are plotted in a color sequence ranging from purple to dark red; data in black arise from other \xt\ vibrational states.  The vertical dashed line separates the rovibrational data (low observation numbers) from the \ax electronic data. ``Weighted Obs-Calc'' corresponds to the Obs-Calc value divided by the frequency error of the transition. }
    \label{fig:res}
\end{figure}


The full list of parameters is reported in Tables S4 and S5 in the \esi, and a subset of parameters pertaining to the \xt(0$v_2$0) levels is reported in Table \ref{tab:CtsX0v20} where they are compared to available literature data. Only five parameters could not be determined in the present fit, the energies of five states [\xt(110), \xt(300), \xt(400), \xt(500), \xt(600)] involved each in a single rovibrational transition for which no cross-correlating data exist.


\input{Tables/CtsX000-020}

\section{Prediction of $\nu_2$ hot bands \label{sec:prednu2}} 

The present modeling of \ccc in its electronic ground and \at\ states can be used to predict further transitions not directly observable. This is particularly interesting for the fundamental hot bands of the $\nu_2$ fundamental that remain elusive in the laboratory to date.
Table \ref{tab:predicted FIR} contains lists of predicted transitions for \xt\,(020) -- \xt\,(010) and \xt\,(030) -- \xt\,(020) band systems. 
These transitions have been calculated using \pgo and the final set of parameters reported in Table \ref{tab:CtsX0v20}.
One limitation of \pgo is that the list of energies does not carry frequency error information, hence we cannot convey these errors to the transitions frequencies. However, based of the frequency errors of the transitions used to determine these energies, and the overall good quality of the fit, we estimate the accuracy of these transition frequencies to be of the order of 0.005~\wn (150 MHz). 


\begin{table}\label{tab:predicted FIR}
\scriptsize
\caption{Low-$J$ far-IR transitions of the \xt\,(020) -- \xt\,(010) and \xt\,(030) -- \xt\,(020) hot bands of $\nu_2$ predicted using our model (in~cm$^{-1}$) } 
\begin{tabular}{l ccc c ccc c ccc}
\toprule
\textbf{$J''$} & \textbf{P} & \textbf{Q} & \textbf{R} && \textbf{P} & \textbf{Q} & \textbf{R} && \textbf{P} & \textbf{Q} & \textbf{R}\\
\midrule

&\multicolumn3c{(020)--(010) $\Sigma-\Pi$} && \multicolumn3c{(020)--(010) $\Delta-\Pi$}\\ \cmidrule{2-4} \cmidrule{6-8}
1 & 68.946 &  & 71.656 &&        & 70.088 &       \\
2 &  & 69.864 &        &&        & 68.295 & 70.088\\
3 & 67.260 &  & 73.588 && 65.692 & 68.411 & 71.014\\
4 &  & 69.959 &        && 64.781 & 68.399 & 72.029\\
5 & 65.678 &  & 75.634 && 64.118 & 68.654 & 72.935\\
6 & & 70.123 &         && 63.143 & 68.547 & 74.058\\


\midrule
& \multicolumn3c{(030)--(020) $\Pi-\Sigma$}  && \multicolumn3c{(030)--(020) $\Pi-\Delta$}  && \multicolumn3c{(030)--(020) $\Phi-\Delta$} \\ \cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12}
0 & &               & 75.075 &&        &        &        && \\
1 & &               &        &&        &        &        && \\
2 & 72.365 & 74.248 & 76.918 && 73.933 & 75.816 & 78.486 &&     &           & 75.842 \\
3 & &               &        && 73.097 & 75.767 & 79.618 &&        & 73.123 & 76.824 \\
4 & 70.590 & 74.440 & 78.788 && 72.150 & 76.000 & 80.348 && 69.505 & 73.207 & 77.831 \\
5 & &               &        && 71.464 & 75.811 & 81.712 && 68.670 & 73.295 & 78.842 \\
6 & 68.831 & 74.732 & 80.682 && 70.408 & 76.309 & 82.258 && 67.891 & 73.439 & 79.903 \\

\bottomrule
\end{tabular}
\end{table}

\section{Astronomical implications \label{sec:astro}} 

Because of the extremely low bending frequency of \ccc , even at a moderate temperature environment, its low excited bending states \xt(010), at $\sim$ 63 \wn / 91\,K,  and \xt(020), at $\sim 132$ \wn / 191 K, can be thermally populated significantly.
Indeed, at 100\,K, 29\,\% and 13\,\% of the  GS population lies in each of these states; at 50\,K, these numbers drop down to 14\,\% and 2\,\%, which remains significant for an abundant molecule. Hence, $\nu_2$ hot bands may be detectable in various environments of the interstellar medium where \ccc is abundant.
Unambiguous detections, $i.e.$, beyond the line confusion limit, become possible when astronomical data can be compared to accurate submillimeter laboratory data (with sub-MHz resolution) that will strongly benefit from the predictions made here. Given the accurate parameters derived here, even without such laboratory data it should be possible to identify these $\nu_2$ excited transitions in astronomical data, $e.g.$, using ALMA.
The 0.005 \wn (150 MHz) accuracy of our predictions corresponds to a velocity uncertainty of $ \Delta V $ = 23.6 km s$^{-1} $. 
Since the linewidth of observed spectra of \ccc $\nu_2$ fundamental band in star forming region ranges from 5 to 12 km s$^{-1} $  \citep{Giesen2001, Mookerjea2010, Mookerjea2012,Giesen2020}, we conclude that our data can be used to search for \ccc $\nu_2$ hot bands. 
Measurement of \ccc in excited states and determination of its abundance and excitation temperature may give new insights into the chemistry of its formation and will add further information to derive the origin of small and possibly also longer carbon chains in the ISM. 




\section{Conclusion} \label{sec:conc} 
This work presents the most complete spectroscopic study of \ccc to date.
Through the combination of infrared and optical transitions precise vibrational energies and rotational constants for the low-lying bending modes of \ccc are determined up to $v_2 = 5$, significantly extending our knowledge of the rovibrational manifold of the electronic GS. The measured and predicted transition frequencies presented here can be used in astronomical observations in both the optical, IR, and FIR, increasing the effectiveness of \ccc as a probe of the physical and chemical environment of the target.  \pgo files allowing the full simulation of all known bands of \ax system are given in the \esi so that further improvements of the laboratory spectroscopy of this molecule can be directly incorporated in the model.



\section{Acknowledgments}
This project started independently in 2010 at ISMO, with the FIR measurements at SOLEIL, and in 2017, with the LIF measurements at USTC. At a later stage the data were merged. It  became soon clear that PGOPHER was ideally suited as a tool to fit both datasets simultaneously. Given all involved spectroscopic challenges, we asked Colin for help, and as usual were helped on the spot and far beyond, resulting in a co-authorship. Along the way of finishing this work, Colin sadly passed away. We dedicate this manuscript to his memory. \\
We acknowledge the financial support of the Netherlands Organization for Scientific Research (NWO) through a VICI grant, and the Netherlands Research School for Astronomy (NOVA), the Programme National “Physique et Chimie du Milieu Interstellaire” (PCMI) of CNRS/INSU with INC/INP co-funded by CEA and CNES. Q.Z. acknowledges financial support from the National Natural Science Foundation of China (21773221 and 21727804), the National Key R\&D program of China (2017YFA0303502), and the Fundamental Research Funds for the Central Universities of China (WK2340000078). Part of this work was performed at the SOLEIL facility under the proposal 20100296.

==> sup.tex <==


\begin{table}
\scriptsize
%\tablewidth{0pt}
\caption{\mam{to be removed} Effective Molecular Constants$^a$ (in~cm$^{-1}$) of C$_3$ in the Electronic Ground State ($\tilde{\mathrm{X}}$\,$^1\Sigma^+_\mathrm{g}$.) }
\label{tab:Ground}

\begin{tabular}{ccccccccccc}
\toprule
State & Symmetry & $T_v$ & $B_v$ & $D_v$ & $H_v$ & $L_v$ & $M_v$ & $q$ & $q_J$ & $q_{JJ}$ \\ 
($v_1 v_2\,^l v_3$)						            &  &  &  & $\times10^5$ & $\times10^9$ & $\times10^{12}$ & $\times10^{16}$ & $\times10^2$ & $\times10^6$ & $\times10^{10}$\\
\midrule

(00$^0$0)$^b$ & $\Sigma^+_\mathrm{g}$ & 0.0 & 0.4305723 & 0.1472 & 0.1333 & & &  & & \\
(01$^1$0)$^b$ & $\Pi_\mathrm{u}$ & 63.416529 & 0.4424068 & 0.2361 & 0.267 & & & 0.56939 & -0.869 & 0.27 \\
(02$^2$0) & $\Delta_\mathrm{g}$ & 131.2224(19) & 0.452737(56) & 0.2531(57) & 0.145(16) & & & 0.5034(44) & -0.395(13) & \\
(02$^0$0) & $\Sigma^+_\mathrm{g}$ & 132.7844(14) & 0.451995(72) & 0.2690(82) & 0.210(24) & & &  & & \\
(03$^3$0) & $\Phi_\mathrm{u}$ & 204.7342(49) & 0.462643(37) & 0.292(38) & 0.143(12) & & & 0.4967(20) & -0.3900(72) & \\
(03$^1$0) & $\Pi_\mathrm{u}$ & 207.3932(20) & 0.460601(38) & 0.2863(41) & 0.226(13) & & & & & \\
(04$^4$0) & $\Gamma_\mathrm{g}$ & 280.5* & 0.471883(23) & 0.3369(25) & 0.200(8) & & & 0.4885(8) & -0.3685(31) & \\
(04$^2$0) & $\Delta_\mathrm{g}$ & 285.3390(14) & 0.468929(26) & 0.2929(27) & 0.181(9) & & & & & \\
(04$^0$0) & $\Sigma^+_\mathrm{g}$ & 286.5644(29) & 0.468074(30) & 0.2744(38) & 0.133(14) & & & & & \\
(05$^5$0) & H$_\mathrm{u}$ & 363.0* & 0.480336(60) & 0.3591(44) & 0.5$^c$ & & & 0.4965(16) & -0.4$^c$ & \\
(05$^3$0) & $\Phi_\mathrm{u}$ & 368.1813(33) & 0.476937(24) & 0.3365$^c$ & 0.5$^c$ & & & & & \\
(05$^1$0) & $\Pi_\mathrm{u}$ & 370.4079(27) & 0.475829(68) & 0.4008(72) & 0.5$^c$ & & & & & \\
(06$^0$0) & $\Sigma^+_\mathrm{g}$ & 460.338(66) & 0.485577(484) & 0.5$^c$ & 0.5$^c$ & & & & & \\
\hline
(00$^0$1) & $\Sigma^+_\mathrm{u}$ & 2040.0216(6) & 0.435656(20) & 0.4236(23) & 0.916(12) & -0.1441(30) & 0.1032(31) & & & \\
(01$^0$1) & $\Pi_\mathrm{g}$ & 2078.4948(81) & 0.454015(18) & 0.5957(21) & 1.026(11) & -0.1306(27) & 0.0786(27) & & & \\
(02$^2$1) & $\Delta_\mathrm{u}$ & 2125.5527(84) & 0.461174(55) & 0.4630(53) & 0.372(15) & & & 0.6373(44) & -0.629(14) & \\
(02$^0$1) & $\Sigma^+_\mathrm{u}$ & 2133.8814(112) & 0.456569(70) & 0.3425(79) & 0.220(23) &  & & & & \\
(03$^3$1) & $\Phi_\mathrm{g}$ & 2180.8891(165) & 0.471583(37) & 0.4846(39) & 0.343(12) & & & 0.6038(20) & -0.5720(70) & \\
(03$^1$1) & $\Pi_\mathrm{g}$ & 2192.7078(165) & 0.465462(39) & 0.3542(40) & 0.227(13) & & & & & \\
(04$^4$1) & $\Gamma_\mathrm{u}$ & 2240.0* & 0.481029(23) & 0.5116(25) & 0.369(8) & & & 0.5706(8) & -0.4848(30) & \\
(04$^2$1) & $\Delta^+_\mathrm{u}$ & 2255.4682(97) & 0.474334(24) & 0.3704(26) & 0.214(9) & & & & & \\
(04$^0$1) & $\Sigma_\mathrm{u}$ & 2260.4349(137) & 0.472022(28) & 0.3130(37) & 0.109(14) & & & & & \\
(05$^5$1) & H$_\mathrm{g}$ & 2307.5* & 0.489554(59) & 0.5156(44) & 0.6$^c$ & & & 0.5600(18) & -0.4$^c$ & \\
(05$^3$1) & $\Phi_\mathrm{g}$ &  2323.8934(233) & 0.482820(29) & 0.4143$^c$ & 0.5$^c$ & & & & & \\
(05$^1$1) & $\Pi_\mathrm{g}$ & 2332.0279(233) & 0.479791(57) & 0.4397(61) & 0.4$^c$ & & & & & \\
\end{tabular}

\begin{minipage}{0.9\textwidth}
$^a$ {Values in parenthesis denote one standard deviation and apply to the last digits of the constants. \textit{l}-type doubling and \textit{l}-type resonance terms ($q$, $q_J$, and $q_{JJ}$) are shared between states of the same $v_2$.}\\
$^b$ {From Ref. \citet{Schmuttenmaer1990}.}\\
$^c$ {Fixed values in the fit \mam{why these values?}}
\end{minipage}

\label{Tab:RotationFitResults}
\end{table}




\newpage


\begin{table}[ht!]
\caption{Molecular constants$^a$ (in~cm$^{-1}$) of C$_3$ in the $\tilde{\mathrm{A}} ^1\Pi_u$ electronic state \mam{P1 P2 P3 are unclear to me} }
\label{tab:Excited}
\begin{tabular}{l c l l l l l}
%\tabletypesize{\scriptsize}
%\tablewidth{0pt}
\toprule
{($v_1 v_2\,^l v_3$)} & {State} & {$\nu_0$} & {$B_v$}                        & {$D_v$}          & {$H_v$} & {q}  \\ 
{}                                                    & {Symmetry} & {}       & {} & {$\times$10$^7$} & {$\times$10$^9$} & {$\times$10$^3$} \\
\midrule
(00$^1$0)$^{b}$ & $\Pi^-_\mathrm{u}$ & 24675.5937(36) & 0.412746(44) & 10.2(3) & 0.13(6) & 0.688(30) \\
P1$^{c,d}$ & $\Sigma^-_\mathrm{g}$ & 24679.757(6) & 0.4439(14) & 9.05(63)$\times$10$^2$ & 1.68(11)$\times$10$^2$ & \\
P2$^c$ & $\Pi_\mathrm{u}$(e) & 24675.72(1) & 0.3487(6) & & & \\
P3$^c$ & $\Pi_\mathrm{u}$(f) & 24675.14(3) & 0.3083(15) & & & \\
(01$^0$0) & $\Sigma^-_\mathrm{g}$ & 24812.2136(8) & 0.415921(12) & 1.39(36) & & \\
(01$^2$0) & $\Delta_\mathrm{g}$ & 24935.0769(5) & 0.415298(6) & 3.28(11) &  & \\
(01$^0$0) & $\Sigma^+_\mathrm{g}$ & 25156.5901(8) & 0.408344(13) & 1.62(39) & & \\
(02$^1$0) & $\Pi^-_\mathrm{u}$ & 25038.5656(9) & 0.418483(24) & 1.04(35) & & 3.83(1)  \\
(02$^1$0) & $\Pi^+_\mathrm{u}$ & 25528.9418(7) & 0.414196(18) & 5.43(83) & & -4.63(1)  \\
(04$^1$0) & $\Pi^-_\mathrm{u}$ & 25440.9558(7) & 0.422564(18) & 14.1(8) & & 5.81(1) \\
(04$^1$0) & $\Pi^+_\mathrm{u}$ & 26297.1187(8) & 0.423004(63) & 21(6) & & 1.62(20) \\
(10$^0$0) & $\Pi_\mathrm{u}$ & 25761.3241(7) & 0.409677(18) & 1.93(77) & & 0.523(11) \\
(00$^0$2) & $\Pi_\mathrm{u}$ & 26346.1441(7) & 0.407349(59) & 46(9) & 22(3) & 0.541(18) \\
(12$^1$0) & $\Pi^-_\mathrm{u}$ & 26127.2303(7) & 0.415403(15) & 3.45(65) & & 3.656(9) \\
\end{tabular}
\begin{minipage}{0.9\textwidth}
$^a$ {Values in parenthesis denote one standard deviation and apply to the last digits of the constants.}\\
$^b$ {Interaction constants are given in the text.}\\
$^b$ {P1, P2, and P3 represent unidentified perturbing states that interaction with $\tilde{\mathrm{A}}$(00$^1$0). \kddcomm{the phrasing of this needs work} }\\
$^d$ {Additional spectroscopic parameters: $\lambda_{ss}$ = -0.1 and $\gamma$ = 1.288(8).}
\end{minipage}

\label{Tab:BandCenterResults}
\end{table}





%\subsection{The $\tilde{\mathrm{A}}$\,(00$^1$0) - $\tilde{\mathrm{X}}$\,(00$^0$0) Bands of $^{13}$C Mono-substituted Isotopologues}

%\begin{deluxetable*}{l c l l l l l}
%    \label{tab:ISO}
%	\tabletypesize{\scriptsize}
%	\tablecaption{The Effective Molecular Constants$^a$ (in~cm$^{-1}$) of $^{13}$C Mono-substituted C$_3$ Isotopologues Origin Band$^b$ }
%	\tablehead{
%	&\\
%		{Isotopologue} & {State} & {G$_v$} & {B$_v$} & {D$_v$} & {H$_v$} &  {q} \\ 
%		{} & {Symmetry} & {} & {} & {$\times$10$^6$} & {$\times$10$^9$} & {$\times$10$^4$} }
%	\startdata
%	$^{12}$C $^{13}$C $^{12}$C & $\tilde{\mathrm{X}}$ $\Sigma^+_g$ & 0.0 & 0.430276 & 1.30 & & \\
%	$^{13}$C $^{12}$C $^{12}$C & $\tilde{\mathrm{X}}$ $\Sigma^+_g$ & 0.0 & 0.413741 & 1.394 & 0.129 & \\
%	\hline
%	$^{12}$C $^{13}$C $^{12}$C & $\tilde{\mathrm{A}}$ $\Pi_u$ & 24684.2782(4) & 0.4123183(42) & 0.1490(83) & & 3.141(17) \\
%	$^{13}$C $^{12}$C $^{12}$C & $\tilde{\mathrm{A}}$ $\Pi_u$ & 24677.8050(3) & 0.3964243(52) & 0.214(12) & & 0.304(58) \\
%	\enddata
%	$^a$ {Values in parenthesis denote one standard deviation and apply to the last digits of the constants.}
%	$^b$ {From \citet{Krieg2013}.}
%\end{deluxetable*}

%\indent In addition to the strong rovibronic features of the normal isotopologue of C$_3$, weak features consistent with transitions expected for the $\tilde{\mathrm{A}}$\,(00$^1$0) - $\tilde{\mathrm{X}}$\,(00$^0$0) bands of the two $^{13}$C mono-substituted isotopologues, $^{13}$CCC and C$^{13}$CC, are recorded. The observed band origins agree well with previous values for the two isotopologues determined by \citet{Haddad2014}, 24677.7849(53)~cm$^{-1}$ and 24684.3048(93)~cm$^{-1}$, respectively. The $^{13}$C mono-substituted isotopologues are produced along with the normal C$_3$ isotopologue in the plasma discharge of the C$_2$H$_2$/Ar gas mixture, which includes $^{13}$C C$_2$H$_2$ at natural abundance. Although the production of the mono-substituted C$_3$ is lower than $^{12}$C$_3$ by almost two orders of magnitude, the S/N of the LIF spectrum is sufficient to perform rotational analysis. This is likely due to the high production efficiency by discharge, the high detection sensitivity of LIF, and the $\tilde{\mathrm{A}}$ - $\tilde{\mathrm{X}}$ transition dipole momentum is large. However, the other three isotopologues ($^{13}$C$^{12}$C$^{13}$C, $^{13}$C$^{13}$C$^{12}$C, $^{13}$C$^{13}$C$^{13}$C) could not be observed in the experimental spectrum; the abundance is expected to be lower than the normal isotopologue by four to six orders of magnitude. \\
%\indent The two isotopologues can be clearly distinguished by the observed line spacing. For the $^{13}$CCC isotopologue, because the two outer C are no longer equivalent (the molecule is not longer centrosymmetric), and the spin statistics no longer gives a 1:0 line intensity alternation. As such, transitions from ground state odd-$J''$ levels are also present, resulting in a narrower line spacings ($\sim$ 2B) compared to that for C$^{13}$CC and $^{12}$C$_3$ ($\sim$ 4B). The narrower spacing is observed in the experimental spectrum suggesting the assignment of $^{13}$C mono-substituted isotopologues to the weak transitions is correct. Accurate band origins and spectroscopic constants are determined from least-square fitting of the observed transitions. The resulting spectroscopic constants are given in Table~\ref{tab:ISO}, including B$'_{^{13}CCC}$ = 0.3964243(52)~cm$^{-1}$ and B$'_{C^{13}CC}$ = 0.4123183(42)~cm$^{-1}$ and agree well with the values determined by \citet{Haddad2014}, B$'_{^{13}CCC}$ = 0.39718(52)~cm$^{-1}$ and B$'_{C^{13}CC}$ = 0.4123(10)~cm$^{-1}$. In addition, confirming the molecular and vibrational assignment, the present rotational constants offer improved precision. In contrast to the severe perturbations seen in the $\tilde{\mathrm{A}}$\,(00$^1$0) state of $^{12}$C$_3$, no perturbations are observed for either monosubstituted isotopologue, and high-$J''$ transitions can be estimated from the determined spectroscopic parameters. Line lists and o-c values for the observed transitions are given in \textbf{supplementary material}; the o-c deviations of all the lines are within 0.002~cm$^{-1}$, well below our experiment accuracy.


\subsection{Combined fit \label{sec:fit}}

\mam{to incorporate: for X (010)}
In these conditions, our set of parameters agrees well with the recent results from \citet{Krieg2013}. For the low- and medium-$J''$ values, the rovibrational energies of the $\tilde{\mathrm{X}}$\,(01$^1$0) manifold obtained from our fit agree with the energies calculated from the results of \citet{Krieg2013}. However, the two energy ladders diverge in the high-$J''$ range (the discrepancy reaches values as high as 0.60~cm$^{-1}$ for $J''$ = 54), likely due to the an under representation of high-$J''$ transitions in the previous study.

\mam{to incorporate: for X (020)}
Thanks to the relatively important extension of the dataset, our fitted upper and lower states rotational constants (presented in table Table~\ref{Tab:RotationFitResults}) are more accurate than previous values from \cite{kawaguchi_diode_1989} and \cite{Krieg2013}. \qiang{Harold's comment: Probably fair to mention how much more; incremental or substantial ?} 

Rotational constants of $\tilde{\mathrm{X}}$ in both $v_3=0$ and $v_3=1$ have been determined from a least-squares-fit of the infrared transitions assuming approximate vibrational energies** \mam{the footnote is missing}.  We used a standard rovibrational Hamiltonian for linear molecules including \textit{l}-type doubling and \textit{l}-type resonance terms, with identical on- and off-diagonal matrix elements as in \citet{Maki1970} and \citet{Schroder2016}, which gives the following on-diagonal term for the rovibrational energy levels:
\begin{equation}\label{eq:upperstate}
\bra{v,J,l} H_{eff} \ket{v,J,l} =  G_v + B_v[J(J + 1)-l^2] - D_v[J(J + 1)-l^2]^2 + H_v[J(J + 1)-l^2]^3
\end{equation}
and off-diagonal term:
\begin{multline}\label{eq:lres}
\bra{v,J,l} H_{eff} \ket{v,J,l \pm 2} =  \frac{1}{4} \left(q + q_JJ(J+1) + q_{JJ}[J(J+1)]^2\right) \\ \times \sqrt{\left[(v_2 + 1)^2 - (l \pm 1)^2\right][J(J+1) - l(l \pm 1)][J(J+1) - (l \pm 1)(l \pm 2)]}
\end{multline}
where $J$ is the total angular momentum quantum number; G$_v$ is the vibrational energy of state $v$; $B_v$, $D_v$, and $H_v$ are the rotational constants and centrifugal distortion terms; and $q_v$, $q_{Jv}$, and $q_{JJv}$ are the rotational \textit{l}-type doubling and \textit{l}-type resonance constants for $l \neq0$ states and the plus and minus signs denote the f and e parity states, respectively. Rotational constants are given in Table \ref{tab:Ground}.

We present in the following paragraphs the details of the rotational analyses of the optical spectra and IR spectra in the section~\ref{sec:optical RA} and \ref{sec:IR RA}, respectively. 

\section{Astrophysical Implications} \label{sec:diss}

\qiang{TBD}
The bending vibration transitions in ground state can be calculated immediately from the rovibrational level energies provided in Table \ref{tab:predicted FIR}. For instance, the far-IR transition frequencies of the $\tilde{\mathrm{X}}$(02$ ^{0/2} $0) - $\tilde{\mathrm{X}}$(01$^1$0), and $\tilde{\mathrm{X}}$(03$^1$0) – $\tilde{\mathrm{X}}$(02$ ^{0} $0) bands are provided in Tables \ref{tab:far-IR-optical}. The accuracy of these transition frequencies is estimated to be $\sim$0.005~\wn, which comes from the uncertainties of the level energies.



\cthree is a pure carbon chain molecule that has been identified in star forming regions and in stellar shells of carbon-rich late-type stars \citep{giesen_interstellar_2001,mookerjea_excitation_2010,mookerjea_chemistry_2012,giesen_first_2020}. Measurement of its abundance and excitation temperature can give insight into the chemistry of its formation in such dense regions.
\cthree molecule has an extremely low bending frequency ($\sim$ 63 \wn). Even at a moderate temperature of \textcolor{red} {50 K} environment, its bending states $\nu_2$ = 1 (E$ _1 $ = 91 K) and $\nu_2$ = 2 (E$ _2 $ =191 K) can be thermally populated significantly. Therefore, the $\nu_2$ hot bands (such as X02$ ^{0/2} $0-X010 and X030-X02$ ^{0/2} $0) are expected to be observable. 
Here we present the far-IR transition line list of \cthree $\nu_2$ hot bands and the accurate constants for the $\nu_2$ levels. The data accuracy is about 0.005 \wn (150 MHz), which is limited by the residual Doppler broadening in our spectra. The 150 MHz accuracy corresponds to a velocity uncertainty of $ \Delta V $ = 23.6 km s$^{-1} $. 
The linewidth of observed spectra of \cthree $\nu_2$ fundamental band in star forming region ranges from 5 to 12 km s$^{-1} $  \citep{giesen_interstellar_2001,mookerjea_excitation_2010,mookerjea_chemistry_2012,giesen_first_2020}.
Based on the above considerations, we conclude that our data can be used to search for \cthree $\nu_2$ hot bands. 

It has been shown that along several translucent sight lines the observed \cthree column densities is well correlated with the corresponding C$ _2 $ column densities and concluded that \cthree and C$ _2 $ are formed in the same chain of chemical reactions \citep{oka_observations_2003}.
However, this chemical pathway can not be used to explain the abundance of \cthree in the warm envelopes of hot cores. 
A gas and grain warm-up model has been used by  \citet{mookerjea_excitation_2010,mookerjea_chemistry_2012} to explain the abundance of \cthree and associated hydrocarbons and give satisfactory results for a few sources at a moderate temperature. 
Further observations of high density warm regions are needed to clearly establish this hypothesis of carbon chain formation in these regions. Consequently, the accurate laboratory data are expected to be helpful.
\qiang{Harold's comment on table 5: Important to list uncertainties here. For astronomers it may be most helpful to provide a Table with calculated line positions. }

\begin{table}[ht!]
\scriptsize
\caption{Predicted far-IR Transitions (in~cm$^{-1}$) of C$_3$}
\label{tab:predicted FIR}
\begin{tabular}{l l l l}
\toprule
{$J''$} & {P} & {Q} & {R} 
\midrule
\multicolumn{4}{c}{(02$^0$0) - (01$^1$0)}\\
1 & 68.933 &  & 71.646 \\
2 &  & 69.859 &  \\
3 & 67.251 &  & 73.580 \\
4 &  & 69.956 &  \\
5 & 65.669 &  & 75.628 \\
\hline
\multicolumn{4}{c}{(03$^1$0) - (02$^0$0)}  \\
0 & & & 75.085 \\
2 & 72.371 & 74.250 & 76.921 \\
4 & 70.592 & 74.445 & 78.791 \\
\end{tabular}
\end{table}

\newpage
\section{Conclusion} \label{sec:conc} %about 1 paragraph
\qiang{TBD}
Through the combination of infrared and optical transitions precise vibrational energies and rotational constants for the low-lying bending modes of C$_3$ were determined up to $\nu_2$ = 6, significantly extending our knowledge of the rovibrational manifold of the electronic ground state. The measured and predicted transition frequencies presented here can be used in astronomical observations in both the optical, IR, and FIR, increasing the effectiveness of C$_3$ as a probe of the physical and chemical environment of the target.  
\qiang{Harold's commment: I guess here the astronomical section could benefit from, by explicitly indicating which info in this ms is now available to search for new C3 transitions in space, summarizing the work already realized so far. Indeed, cover optical work (Schmidt et al), IR (check with work Giesen) and in the FIR, where only the v0-1 has been seen, as far as I know. }


